UCTopic: Unsupervised Contrastive Learning for Phrase Representations and Topic Mining

High-quality phrase representations are essential to finding topics and related terms in documents (a.k.a. topic mining). Existing phrase representation learning methods either simply combine unigram representations in a context-free manner or rely on extensive annotations to learn context-aware knowledge. In this paper, we propose UCTopic, a novel unsupervised contrastive learning framework for context-aware phrase representations and topic mining. UCTopic is pretrained in a large scale to distinguish if the contexts of two phrase mentions have the same semantics. The key to pretraining is positive pair construction from our phrase-oriented assumptions. However, we find traditional in-batch negatives cause performance decay when finetuning on a dataset with small topic numbers. Hence, we propose cluster-assisted contrastive learning(CCL) which largely reduces noisy negatives by selecting negatives from clusters and further improves phrase representations for topics accordingly. UCTopic outperforms the state-of-the-art phrase representation model by 38.2% NMI in average on four entity cluster-ing tasks. Comprehensive evaluation on topic mining shows that UCTopic can extract coherent and diverse topical phrases.

==> 0_abstract.tex <==
% \begin{abstract}
% Topic mining aims to find topics and related terms in documents. Previous works 
% %cannot handle phrases well 
% struggle to handle phrases well
% due to the absence of effective phrase representations. In this paper, we present \our, a contrastive learning framework that 
% %greatly 
% advances 
% %the 
% phrase representation and topic mining. We first propose two hypotheses of phrases to produce noise for contrastive learning, with only masking words in the sentences. Based on the two hypotheses, we pre-train a backbone model with a contrastive objective. Then, to finetune and learn data-specific topics, we propose cluster-assisted contrastive learning which utilizes pseudo-labels from clustering to provide hard negatives and further improves phrase representations for topics accordingly. 
% By 
% %objective 
% evaluation on entity clustering, 
% We find \our outperforms state-of-the-art 
% %model of 
% phrase representation models by $38.2\%$ NMI in average. 
% Comprehensive evaluation on topic modeling shows that \our can extract coherent and diverse topical phrases.

%\end{abstract}


\begin{abstract}

\jingbo{
I think the major contribution here is a new pre-training task for phrase representation learning. 
The existing entity/phrase representation learning method LUKE requires a large amount of known span information (e.g., from wiki hyperlinks) so it cannot be easily generalized to domain-specific text corpora. 
So why the title is centered at phrase topic mining?
What's phrase topic mining? Or it's topic phrase mining?
Shall we change the title to something related to phrase representation learning and then position phrase topic mining as an evaluation task?
}

\jingbo{
Let's try this flow and see if it's better:
(1) What's topic mining and why it's important to have high-quality phrase representations.
(2) While unsupervised MLM has been developed for unigram representation learning, when it comes to phrases, it still requires some annotations (e.g., LUKE's case).
(3) Towards better topic mining in domain-specific corpora (mainly to lift the requirement on annotations), we propose a novel phrase representation learning based on unsupervised contrastive learning.
(4) Talk about the pre-training task
(5) Talk about the challenge in the fine-tuning stage and what's the solution.
(6) Mention those empirical evidence. 
}

Topic mining aims to find topics and related terms in documents. 
Phrase representation is essential to understand phrase semantics and extract topics.
\jingbo{How about existing methods for phrase representation learning?}
In this paper, we present \our, a contrastive learning framework that advances phrase representation by a large-scale pre-training without supervision. 
\jingbo{It is not clear here what's the pre-training task. Distinguish if the contexts of two phrase mentions are talking about the same semantic? }
We first propose a phrase-oriented method to constructing training pairs have the same phrase semantics, with only masking words in phrases. 
\jingbo{this ``masking words in phrases'' is confusing. Shall we mention some masked language model earlier?}
Based on training pairs, we pre-train phrase representations with a contrastive objective. 
\jingbo{positive pairs are mentioned but how about negative ones?}
Then, to learn data-specific topics, we propose cluster-assisted contrastive learning (CCL) for finetuning. 
\jingbo{What's this CCL doing? Why it can reduce noise in negatives?}
\jingbo{From the later Figure 2, I feel CCl actually provides more diverse negatives instead of reducing the noise?}
\jingbo{I understand it now after reading intro that the noise is caused by the in-batch negatives. let's make it more explicit here.}
The CCL largely reduces the noisy negatives of contrastive learning and further improves phrase representations for topics accordingly. 
We find \our outperforms state-of-the-art phrase representation models by $38.2\%$ NMI in average on four entity clustering tasks. 
Comprehensive evaluation on topic modeling shows that \our can extract coherent and diverse topical phrases.
\end{abstract}



